Dynamic Sparse Training of Diagonally Sparse Networks

Recent advances in Dynamic Sparse Training (DST) have pushed the frontier of sparse neural network training in structured and unstructured contexts, matching dense-model performance while drastically reducing parameter counts to facilitate model scaling. However, unstructured sparsity often fails to translate into practical speedups on modern hardware. To address this shortcoming, we propose DynaDiag, a novel structured sparse-to-sparse DST method that performs at par with unstructured sparsity. DynaDiag enforces a diagonal sparsity pattern throughout training and preserves sparse computation in forward and backward passes. We further leverage the diagonal structure to accelerate computation via a custom CUDA kernel, rendering the method hardware-friendly. Empirical evaluations on diverse neural architectures demonstrate that our method maintains accuracy on par with unstructured counterparts while benefiting from tangible computational gains. Notably, with 90% sparse linear layers in ViTs, we observe up to a 3.13x speedup in online inference without sacrificing model performance and a 1.59x speedup in training on a GPU compared to equivalent unstructured layers. Our source code is available at https://github.com/horizon-research/DynaDiag/.

==> background.tex <==
\section{Background}
\label{sec:background}
\fixme{In this section, we first describe the tradeoffs associated with structure and unstructured neural networks (~\Sect{sec:bkg:strucunstruc}). We then describe the two categories of sparse training (~\Sect{sec:bkg:dsst}).}

\subsection{Structured and Unstructured Sparsity}
\label{sec:bkg:strucunstruc}
- why study sparse training? What are the ideal goals of a sparse training method?
- What is the meaning of struc and unstruc? \\
- What are the tradeoffs in algorithmic vs system level performance?
\subsection{Dynamic and Static Sparse Training}
\label{sec:bkg:dsst}
%- Explain DST: what is it? advantages? disadvantages? Challenges\\
\paragraph{Dynamic Sparse Training} produces sparse neural networks by changing the 
- Explain SST: what is it? advantages? disadvantages? Challenges

